Strategic Prediction with Latent Aggregative Games

We introduce a new class of context dependent, incomplete information games to serve as structured prediction models for settings with significant strategic interactions. Our games map the input context to outcomes by first condensing the input into private player types that specify the utilities, weighted interactions, as well as the initial strategies for the players. The game is played over multiple rounds where players respond to weighted aggregates of their neighbors' strategies. The predicted output from the model is a mixed strategy profile (a near-Nash equilibrium) and each observation is thought of as a sample from this strategy profile. We introduce two new aggregator paradigms with provably convergent game dynamics, and characterize the conditions under which our games are identifiable from data. Our games can be parameterized in a transferable manner so that the sets of players can change from one game to another. We demonstrate empirically that our games as models can recover meaningful strategic interactions from real voting data.

==> RehnquistCourt.tex <==
\begin{tikzpicture}[shorten >=1pt, auto, thick,
        node distance=0.6cm,
    con node/.style={circle,draw,fill=red!20,font=\sffamily\Large\bfseries},
    lib node/.style={circle,draw,fill=blue!20,font=\sffamily\Large\bfseries},
    mod node/.style={circle,draw,fill=green!20,font=\sffamily\Large\bfseries}] 
    
   
%\node[main node, label={above:\small Kennedy}] (KA) {$K$};
% \node[main node, left=of KA, yshift=1cm, label={above: \small Alito}]     (AA)   {$A$};
% \node[main node, left=of AA,  label={above: \small Thomas}]     (TA)   {$T$};
% \node[main node, below=of TA,  label={below: \small Scalia}]     (SA)   {$S$};  
% \node[main node, below=of AA,  label={below: \small Roberts}]     (RA)   {$R$};
% \node[main node, right=of KA, yshift=1cm, label={above: \small Ginsburg}]     (GA)   {$G$};
% \node[main node, below=of GA,  label={below: \small Breyer}]     (BA)   {$B$};
% \foreach \from/\to in {AA/TA, AA/RA, RA/AA, SA/RA, TA/SA, AA/KA, GA/KA, GA/BA, BA/GA}
% \draw[-latex] (\from) edge (\to);  
%\plate{Conservatives}{(AA)(TA)(RA)(SA)}{\bf Conservatives};
%\plate{Liberals}{(BA)(GA)}{\bf Liberals};

\node[mod node] (KL) {$K$};
 \node[con node, left=of KL, yshift=-2cm]     (RL)   {$R$};
 \node[con node, left=of RL, yshift= 1cm]     (ScL)   {$Sc$};
 \node[con node, left=of RL, yshift= -1cm]    (TL)   {$T$};
 \node[mod node, right=of RL, yshift= -1cm]     (OL)   {$O$};
 \node[lib node, right=of KL, yshift = -1cm]     (GL)   {$G$};
 \node[lib node, right=of GL]     (SoL)   {$So$};
 \node[lib node, below=of GL]     (BL)   {$B$};
 \node[lib node, below=of SoL]     (StL)   {$St$};
 \foreach \from/\to in {RL/ScL, TL/RL, ScL/TL, TL/ScL, RL/KL, RL/OL, GL/KL, GL/BL, BL/OL,  SoL/GL, GL/StL, StL/SoL, SoL/BL, BL/GL}
 \draw[-latex] (\from) edge (\to);  
 
\draw (TL) -- node [below=1.5 cm, xshift=2cm] {{\bf (a)\,\, Positive\, Influence}} (RL);

\node[mod node, right=of SoL, xshift = 2cm, yshift = 0.5cm]  (KR) {$K$}; 
\node[con node, right=of KR, yshift = 0.8cm]  (ScR) {$Sc$}; 
\node[mod node, right=of ScR, xshift = 0.8cm]  (OR) {$O$};
\node[lib node, right=of KR, xshift = 2.3cm, yshift =-0.3cm]  (StR) {$St$}; 
\node[lib node, below=of KR, yshift = 0.2cm]  (SoR) {$So$}; 
\node[con node, below=of StR, yshift=0.4cm]  (RR) {$R$}; 
\node[lib node, below=of RR]  (BR) {$B$}; 
\node[con node, below=of SoR, xshift=0.2cm, yshift = 0.2cm]  (TR) {$T$};
\node[lib node, right=of TR]  (GR) {$G$}; 
 \foreach \from/\to in {ScR/KR, ScR/OR, ScR/SoR, SoR/OR, SoR/TR, StR/TR, StR/KR,  StR/ScR, ScR/GR, BR/ScR, RR/BR, BR/RR, RR/GR}
 \draw[-latex] (\from) edge [magenta](\to); 

\draw[magenta] (SoR) -- node [yshift = -2cm, color=black] {{\bf (b)\,\, Negative\, Influence}} (TR);
%
%
%
%
%
%
%\node[main node, right=of KA, xshift = 5.5cm]     (K)   {$K$};
%\node[main node, left=of K, yshift = 1cm]     (A)   {$A$};
%\node[main node, left=of K, yshift = -0.7cm]     (S)   {$S$};
%\node[main node, left=of S]     (R)   {$R$};
%\node[main node, above=of R]     (T)   {$T$};
%\node[main node, right=of K, yshift= -0.7cm]    (B)   {$B$};
%\node[main node, right=of K, yshift= 1cm]     (G)   {$G$};
%
%\foreach \from/\to in {A/T,  A/R, R/A, S/R, T/S, A/K, A/G,  G/K, S/B}
%\draw[-latex] (\from) edge (\to);
%\
%\draw (R) -- node [below=1.6cm, xshift=1.5cm] {${\bf (b)\,\,\gamma-aggregative \,(\ell=2,\,\, \gamma =0.9)}$} (A);
%
\end{tikzpicture}
\endinput

\node[main node, below=3cm of KA] (Kr) {$K$};
 \node[main node, left=of Kr, yshift=1cm]     (Ar)   {$A$};
 \node[main node, left=of Ar]     (Tr)   {$T$};
 \node[main node, below=of Tr]     (Sr)   {$S$};  
 \node[main node, below=of Ar]     (Rr)   {$R$};
 \node[main node, right=of Kr, yshift=1cm]     (Gr)   {$G$};
 \node[main node, below=of Gr]     (Br)   {$B$};
 \foreach \from/\to in {Ar/Tr, Ar/Rr, Rr/Ar, Sr/Rr, Tr/Sr, Ar/Kr, Gr/Kr, Gr/Br, Br/Gr}
 \draw (\from) edge (\to);  
\draw (Rr) -- node [below=1.5cm, xshift=1.5cm] {${\bf (c)\,\, Local \,\,Aggregative \,\,(Undirected \,\, \& \,\, Relaxed)}$} (Ar);

%\node[main node, below=3cm of KA]     (Kr)   {$K$};
%\node[main node, left=of Kr, yshift = 1cm]     (Rr)   {$R$};
%\node[main node, left=of Kr, yshift = -0.7cm]     (Sr)   {$S$};
%\node[main node, left=of Rr]     (Tr)   {$T$};
%\node[main node, left=of Sr]     (Ar)   {$A$};
%\node[main node, right=of Kr, yshift= -0.7cm]    (Br)   {$B$};
%\node[main node, right=of Kr, yshift= 1cm]     (Gr)   {$G$};

%\foreach \from/\to in {Tr/Ar, Ar/Rr, Sr/Rr, Ar/Kr, Kr/Gr, Gr/Br}
%\draw (\from) edge (\to);



\node[main node, below=3cm of KA, xshift = 7cm]     (Ka)   {$K$};
\node[main node, left=of Ka, yshift = 1cm]     (Ra)   {$R$};
\node[main node, left=of Ka, yshift = -0.7cm]     (Sa)   {$S$};
\node[main node, left=of Ra]     (Ta)   {$T$};
\node[main node, left=of Sa]     (Aa)   {$A$};
\node[main node, right=of Ka, yshift= -0.7cm]    (Ba)   {$B$};
\node[main node, right=of Ka, yshift= 1cm]     (Ga)   {$G$};

\foreach \from/\to in {Ka/Ra}  
\draw (\from) edge (\to);   
\foreach \from/\to in {Ka/Sa}   
\draw (\from) edge (\to);
\foreach \from/\to in {Ka/Ba}   
\draw (\from) edge (\to);
\foreach \from/\to in {Ta/Ra}   
\draw (\from) edge (\to);
\foreach \from/\to in {Ga/Ba}  
\draw (\from) edge (\to);
\foreach \from/\to in {Aa/Sa}  
\draw (\from) edge (\to);

\draw (Aa) -- node [below=0.6cm, xshift=2cm] {${\bf (d)\,\, Potential\,\, Hamming}$} (Sa);

%\plate{Conservatives}{(A)(T)(R)(S)}{\bf Conservatives};
%\plate{Liberals}{(B)(G)}{\bf Liberals};

%\node[wrong node, right= of G, xshift = 2cm]  (T1)  {$T$};
%\node[main node, above=of T1]  (B1)  {$B$};
%\node[main node, left=of T1] (K1) {$K$};
%\node[wrong node, below=of T1] (G1) {$G$};
%\node[main node, right=of T1] (R1) {$R$};
%\node[main node, right=of G1] (S1) {$S$};
%\node[main node, above=of R1] (A1) {$A$};
%\foreach \from/\to in {B1/K1, K1/G1, S1/R1, R1/A1} 
%\path (\from) edge (\to);
%\foreach \from/\to in {T1/B1, G1/S1} 
%\path (\from) edge[red] (\to);

%\draw[red,
%    decoration={markings,mark=at position 1 with {\arrow[scale=4,blue]{>}}},
%    %postaction={decorate},
%    shorten >=0.4pt];
%  \draw [-to,shorten >=-1pt,ultra thick] (-3,2) -- (3,2);   
%  \node[] at (0,2.3) {Increasing Liberalism};
\end{tikzpicture}




 \endinput

{'T', 'R', 'S', 'K', 'G', 'B', 'A'}
  \node[obs]                   (X)      {$x_{nd}$} ; %
  \node[latent, left=of X, xshift=-1cm ]    (Y)      {$v_{kd}$} ; %
  \node[latent, left=of Y]    (nu)      {$\nu_{kd}$} ; %
  \node[latent, left=of nu, xshift= -3.0cm, yshift=1cm]    (M)      {$m$} ; %
 % \node[latent, left=of M, yshift=-0.5cm]    (gamma)      {$\gamma_k$} ;
  % \node[latent, left=of M, yshift=0.5cm]    (delta)      {$\delta_k$} ;
   \node[latent, left=of nu,  xshift= -3.0cm, yshift=-1cm]    (rho)      {$\rho$} ;
   \node[latent, above=of Y, xshift=-4.1cm, yshift=1.2cm]    (eta)      {$\eta_{kdt}$} ;
   \node[obs, above=of X, yshift= 2cm, xshift=0.3cm] (meanGlobal) {$\zeta_{d}$};
   \node[obs, above=of X, yshift= 2cm, xshift=-1cm] (sigmaGlobal) {$\sigma_{d}$};
   \node[latent, above=of X, xshift=-2.6cm, yshift=1.6cm]    (sigma) {$\sigma_{kd}$};
   \node[latent, above=of X, xshift=-2.5cm, yshift=2.5cm ]    (zeta)      {$\zeta_{kd}$} ;
   \node[obs, above=of X, yshift=2.3cm, xshift=1.6cm]    (etad) {$\eta_{0dt}$};
   \node[latent, left=of eta, xshift=1cm] (alpha) {$\alpha_{kdt}$};
   \node[latent, right=of X, yshift=0.6cm, xshift=-0.9cm ]    (Z)      {$z_{n,k}$} ;
   \node[latent, above=of Z, xshift=0.3cm, yshift=-0.4cm]    (theta)      {$\theta$} ; 
   \edge[dashed, ->] {M}{rho};

%\edge{gamma}{M}
%\edge{delta}{M}
\edge{M}{nu}
%\plate{}{(gamma)(delta)(M)}{$\infty$}
\edge{meanGlobal}{X}
\edge{rho}{nu}
\edge{nu}{Y}
\edge{eta}{X}
\edge{etad}{X}
\edge{sigmaGlobal}{X}
 \edge {Y} {X}
 \edge{zeta}{X}
 \edge{Z}{X}
 \edge{sigma}{X}
 \edge{theta}{Z}
 \edge{alpha}{eta}
 \plate{etaT}{(etad)}{$\vert \mathcal{T}_d \vert$}
 \plate{etaTD}{(etaT)}{$|Cat|$}
 \plate{}{(meanGlobal)(sigmaGlobal)}{$\vert Num \vert$}
 \plate{plateNY}{(nu)(Y)}{$D = |Num| + |Cat|$}
 \plate{plateEta}{(eta)(alpha)}{$\vert \mathcal{T}_d \vert$}
 \plate{plateCat}{(plateEta)}{$\vert Cat \vert$}
 \plate{plateZeta}{(zeta)(sigma)}{$\vert Num \vert$}
 \plate{}{(plateNY)(plateCat)(plateZeta)}{$\infty$}
 %\plate{}{(mu)(nu)(Y)}{$D$}
 \plate{plateX}{(X)}{$D$}
 \plate{plateZ}{(Z)}{$\infty$}
\plate{plateZX}{(plateZ)(plateX)}{$N$}
 %\plate{plate1}{(plateEta)(plateZeta)(Y)}{$\infty$}
 
%\plate{}{(nu)(plate1)(X)}{$D = \vert Cat \vert + \vert Num \vert$}

 
 
 \end{tikzpicture}
 
  % Factors
%  \factor[above=of X]     {X-f}     {Multi} {} {} ; %
%  \factor[above=of T]     {T-f}     {left:Multi} {} {} ; %
%  \factor[above=of theta] {theta-f} {left:Dir} {} {} ; %

  
  %\node[const, above=of phi]  (aphi) {$\alpha_\phi$}; %

  %\factor[above=of phi] {phi-f} {right:Dir} {} {} ; %

%%  \factoredge {theta}  {T-f}     {T} ; %
%%  \factoredge {atheta} {theta-f} {theta} ; %
%%  \factoredge {phi}    {X-f}     {X} ; %
%%  \factoredge {aphi}   {phi-f}   {phi} ; %
%%
%%  \gate {X-gate} {(X-f)(X-f-caption)} {T}
%%
%%  \plate {plate1} { %
%%    (X)(X-gate) %
%%    (T)(T-f)(T-f-caption) %
%%  } {$\forall 1 \leq i \leq n_d$}; %
%%  \plate {} { %
%%    (plate1) %
%%    (theta)(theta-f)(theta-f-caption) %
%%  } {$\forall d \in \mathcal{D}$} ; %
%%  \plate {} { %
%%    (phi)(phi-f)(phi-f-caption) %
%%  } {$\forall t \in \mathcal{T}$} ; %
%%
%%\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 


==> RehnquistCourtQuant.tex <==
\begin{tikzpicture}[shorten >=1pt, auto, thick,
        node distance=0.3cm,
    con node/.style={circle,draw,fill=red!20,font=\sffamily\small\bfseries},
    lib node/.style={circle,draw,fill=blue!20,font=\sffamily\small\bfseries},
    mod node/.style={circle,draw,fill=green!20,font=\sffamily\small\bfseries}] 
    
   
%\node[main node, label={above:\small Kennedy}] (KA) {$K$};
% \node[main node, left=of KA, yshift=1cm, label={above: \small Alito}]     (AA)   {$A$};
% \node[main node, left=of AA,  label={above: \small Thomas}]     (TA)   {$T$};
% \node[main node, below=of TA,  label={below: \small Scalia}]     (SA)   {$S$};  
% \node[main node, below=of AA,  label={below: \small Roberts}]     (RA)   {$R$};
% \node[main node, right=of KA, yshift=1cm, label={above: \small Ginsburg}]     (GA)   {$G$};
% \node[main node, below=of GA,  label={below: \small Breyer}]     (BA)   {$B$};
% \foreach \from/\to in {AA/TA, AA/RA, RA/AA, SA/RA, TA/SA, AA/KA, GA/KA, GA/BA, BA/GA}
% \draw[-latex] (\from) edge (\to);  
%\plate{Conservatives}{(AA)(TA)(RA)(SA)}{\bf Conservatives};
%\plate{Liberals}{(BA)(GA)}{\bf Liberals};

\node[mod node] (KL) {$K$};
 \node[con node, left=of KL, yshift=-1cm]     (RL)   {$R$};
 \node[con node, left=of RL, yshift= 1cm]     (ScL)   {$Sc$};
 \node[con node, left=of RL, yshift= -1cm]    (TL)   {$T$};
 \node[mod node, right=of RL, yshift= -1cm]     (OL)   {$O$};
 \node[lib node, right=of KL, yshift = -0.5cm]     (GL)   {$G$};
 \node[lib node, right=of GL]     (SoL)   {$So$};
 \node[lib node, below=of GL]     (BL)   {$B$};
 \node[lib node, below=of SoL]     (StL)   {$St$};
 \foreach \from/\to in {RL/ScL, TL/RL, ScL/TL, TL/ScL, RL/KL, RL/OL, GL/KL, GL/BL, BL/OL,  SoL/GL, GL/StL, StL/SoL, SoL/BL, BL/GL}
 \draw[-latex] (\from) edge (\to);  
 
\draw (TL) -- node [below=1 cm, xshift=1.5cm] {{\bf (a)\,\, LAG\, (Ours)}} (RL);

\node[mod node, right=of KL, xshift = 4.5cm] (KM) {$K$};
 \node[con node, left=of KM, yshift=-1cm, xshift=-0.6cm]     (RM)   {$R$};
 \node[con node, left=of RM, yshift= 1cm, xshift=0.6cm]     (ScM)   {$Sc$};
 \node[con node, left=of RM, yshift= -1cm, xshift=0.6cm]    (TM)   {$T$};
 \node[mod node, right=of RM, yshift= -1cm, xshift=0.6cm]     (OM)   {$O$};
 \node[lib node, right=of KM, yshift = -0.5cm]     (GM)   {$G$};
 \node[lib node, right=of GM]     (SoM)   {$So$};
 \node[lib node, below=of GM]     (BM)   {$B$};
 \node[lib node, below=of SoM]     (StM)   {$St$};
  
\foreach \from/\to in {OM/RM,  ScM/RM, TM/RM, SoM/StM, RM/ScM, OM/ScM, KM/ScM,  BM/SoM, RM/TM, OM/TM, KM/TM, StM/GM, BM/GM, SoM/BM}
\draw[-latex] (\from) edge [black](\to); 

\foreach \from/\to in {BM/StM, KM/OM, OM/KM, ScM/KM, TM/KM, StM/SoM, StM/BM, OM/BM}
\draw[-latex] (\from) edge [red](\to); 




%R: <--- O Sc T
%St: <--- So B
%O: <--- K
%Sc: <--- R O K
%K: <--- O Sc T
%So: <--- St B
%T: <--- R O K
%G: <--- St B
%B: <--- St O So

%R: <--- O Sc T
% St: <--- So
% O: <---
% Sc: <--- R O K
% K: <---
% So: <--- B
% T: <--- R O K
% G: <--- St B
% B: <--- So


\draw (TM) -- node [below=1 cm, xshift=1.5cm] {{\bf (b)\,\, Local\, AG \cite{GJ2017}}} (RM);

\node[mod node, right=of KM, xshift = 4.5cm] (KR) {$K$};
 \node[con node, left=of KR, yshift=-1cm, xshift=-0.3cm]     (RR)   {$R$};
 \node[con node, left=of RR, yshift= 1cm, xshift=0.3cm]     (ScR)   {$Sc$};
 \node[con node, left=of RR, yshift= -1cm, xshift=0.3cm]    (TR)   {$T$};
 \node[mod node, right=of RR, yshift= -1cm, xshift=0.3cm]     (OR)   {$O$};
 \node[lib node, right=of KR, yshift = -0.5cm]     (SoR)   {$So$};
 \node[lib node, right=of SoR]     (GR)   {$G$};
 \node[lib node, below=of SoR]     (StR)   {$St$};
 \node[lib node, below=of GR]     (BR)   {$B$};
 
\foreach \from/\to in {RR/StR,  StR/RR, StR/ScR, ScR/StR,  StR/SoR, SoR/StR, StR/GR, GR/StR, StR/BR, BR/StR, ScR/TR, TR/ScR, OR/KR, KR/OR}
\draw[-latex] (\from) edge [black](\to); 

\foreach \from/\to in {SoR/OR, OR/SoR}
\draw[-latex] (\from) edge [red](\to); 


%\draw (TR) -- node [below=1 cm, xshift=1.5cm] {{\bf (c)\,\, Tree Structured Potential\, Game  [10]}} (RR); 
\draw (TM) -- node [below=1 cm, xshift=7cm] {{\bf (c)\,\, Tree Structured Potential\, Game  \cite{GJ2016}}}  (RM);


% \foreach \from/\to in {ScR/KR, ScR/OR, ScR/SoR, SoR/OR, SoR/TR, StR/TR, StR/KR,  StR/ScR, ScR/GR, BR/ScR, RR/BR, BR/RR, RR/GR}
 
 
 
%R: <--- O Sc T
%St: <--- So B
%O: <--- K
%Sc: <--- R O K
%K: <--- O Sc T
%So: <--- St B
%T: <--- R O K
%G: <--- St B
%B: <--- St O So

%if nargin < 3, beta = 0.01; end
%if nargin < 2, alpha = 1; end
%if nargin < 1, C = 10; end

%\draw[magenta] (SoM) -- node [yshift = -2cm, color=black] {{\bf (b)\,\, Negative\, Influence}} (TM);
%
%
%
%
%
%
%\node[main node, right=of KA, xshift = 5.5cm]     (K)   {$K$};
%\node[main node, left=of K, yshift = 1cm]     (A)   {$A$};
%\node[main node, left=of K, yshift = -0.7cm]     (S)   {$S$};
%\node[main node, left=of S]     (R)   {$R$};
%\node[main node, above=of R]     (T)   {$T$};
%\node[main node, right=of K, yshift= -0.7cm]    (B)   {$B$};
%\node[main node, right=of K, yshift= 1cm]     (G)   {$G$};
%
%\foreach \from/\to in {A/T,  A/R, R/A, S/R, T/S, A/K, A/G,  G/K, S/B}
%\draw[-latex] (\from) edge (\to);
%\
%\draw (R) -- node [below=1.6cm, xshift=1.5cm] {${\bf (b)\,\,\gamma-aggregative \,(\ell=2,\,\, \gamma =0.9)}$} (A);
%
\end{tikzpicture}
\endinput

\node[main node, below=3cm of KA] (Kr) {$K$};
 \node[main node, left=of Kr, yshift=1cm]     (Ar)   {$A$};
 \node[main node, left=of Ar]     (Tr)   {$T$};
 \node[main node, below=of Tr]     (Sr)   {$S$};  
 \node[main node, below=of Ar]     (Rr)   {$R$};
 \node[main node, right=of Kr, yshift=1cm]     (Gr)   {$G$};
 \node[main node, below=of Gr]     (Br)   {$B$};
 \foreach \from/\to in {Ar/Tr, Ar/Rr, Rr/Ar, Sr/Rr, Tr/Sr, Ar/Kr, Gr/Kr, Gr/Br, Br/Gr}
 \draw (\from) edge (\to);  
\draw (Rr) -- node [below=1.5cm, xshift=1.5cm] {${\bf (c)\,\, Local \,\,Aggregative \,\,(Undirected \,\, \& \,\, Relaxed)}$} (Ar);

%\node[main node, below=3cm of KA]     (Kr)   {$K$};
%\node[main node, left=of Kr, yshift = 1cm]     (Rr)   {$R$};
%\node[main node, left=of Kr, yshift = -0.7cm]     (Sr)   {$S$};
%\node[main node, left=of Rr]     (Tr)   {$T$};
%\node[main node, left=of Sr]     (Ar)   {$A$};
%\node[main node, right=of Kr, yshift= -0.7cm]    (Br)   {$B$};
%\node[main node, right=of Kr, yshift= 1cm]     (Gr)   {$G$};

%\foreach \from/\to in {Tr/Ar, Ar/Rr, Sr/Rr, Ar/Kr, Kr/Gr, Gr/Br}
%\draw (\from) edge (\to);



\node[main node, below=3cm of KA, xshift = 7cm]     (Ka)   {$K$};
\node[main node, left=of Ka, yshift = 1cm]     (Ra)   {$R$};
\node[main node, left=of Ka, yshift = -0.7cm]     (Sa)   {$S$};
\node[main node, left=of Ra]     (Ta)   {$T$};
\node[main node, left=of Sa]     (Aa)   {$A$};
\node[main node, right=of Ka, yshift= -0.7cm]    (Ba)   {$B$};
\node[main node, right=of Ka, yshift= 1cm]     (Ga)   {$G$};

\foreach \from/\to in {Ka/Ra}  
\draw (\from) edge (\to);   
\foreach \from/\to in {Ka/Sa}   
\draw (\from) edge (\to);
\foreach \from/\to in {Ka/Ba}   
\draw (\from) edge (\to);
\foreach \from/\to in {Ta/Ra}   
\draw (\from) edge (\to);
\foreach \from/\to in {Ga/Ba}  
\draw (\from) edge (\to);
\foreach \from/\to in {Aa/Sa}  
\draw (\from) edge (\to);

\draw (Aa) -- node [below=0.6cm, xshift=2cm] {${\bf (d)\,\, Potential\,\, Hamming}$} (Sa);

%\plate{Conservatives}{(A)(T)(R)(S)}{\bf Conservatives};
%\plate{Liberals}{(B)(G)}{\bf Liberals};

%\node[wrong node, right= of G, xshift = 2cm]  (T1)  {$T$};
%\node[main node, above=of T1]  (B1)  {$B$};
%\node[main node, left=of T1] (K1) {$K$};
%\node[wrong node, below=of T1] (G1) {$G$};
%\node[main node, right=of T1] (R1) {$R$};
%\node[main node, right=of G1] (S1) {$S$};
%\node[main node, above=of R1] (A1) {$A$};
%\foreach \from/\to in {B1/K1, K1/G1, S1/R1, R1/A1} 
%\path (\from) edge (\to);
%\foreach \from/\to in {T1/B1, G1/S1} 
%\path (\from) edge[red] (\to);

%\draw[red,
%    decoration={markings,mark=at position 1 with {\arrow[scale=4,blue]{>}}},
%    %postaction={decorate},
%    shorten >=0.4pt];
%  \draw [-to,shorten >=-1pt,ultra thick] (-3,2) -- (3,2);   
%  \node[] at (0,2.3) {Increasing Liberalism};
\end{tikzpicture}




 \endinput

{'T', 'R', 'S', 'K', 'G', 'B', 'A'}
  \node[obs]                   (X)      {$x_{nd}$} ; %
  \node[latent, left=of X, xshift=-1cm ]    (Y)      {$v_{kd}$} ; %
  \node[latent, left=of Y]    (nu)      {$\nu_{kd}$} ; %
  \node[latent, left=of nu, xshift= -3.0cm, yshift=1cm]    (M)      {$m$} ; %
 % \node[latent, left=of M, yshift=-0.5cm]    (gamma)      {$\gamma_k$} ;
  % \node[latent, left=of M, yshift=0.5cm]    (delta)      {$\delta_k$} ;
   \node[latent, left=of nu,  xshift= -3.0cm, yshift=-1cm]    (rho)      {$\rho$} ;
   \node[latent, above=of Y, xshift=-4.1cm, yshift=1.2cm]    (eta)      {$\eta_{kdt}$} ;
   \node[obs, above=of X, yshift= 2cm, xshift=0.3cm] (meanGlobal) {$\zeta_{d}$};
   \node[obs, above=of X, yshift= 2cm, xshift=-1cm] (sigmaGlobal) {$\sigma_{d}$};
   \node[latent, above=of X, xshift=-2.6cm, yshift=1.6cm]    (sigma) {$\sigma_{kd}$};
   \node[latent, above=of X, xshift=-2.5cm, yshift=2.5cm ]    (zeta)      {$\zeta_{kd}$} ;
   \node[obs, above=of X, yshift=2.3cm, xshift=1.6cm]    (etad) {$\eta_{0dt}$};
   \node[latent, left=of eta, xshift=1cm] (alpha) {$\alpha_{kdt}$};
   \node[latent, right=of X, yshift=0.6cm, xshift=-0.9cm ]    (Z)      {$z_{n,k}$} ;
   \node[latent, above=of Z, xshift=0.3cm, yshift=-0.4cm]    (theta)      {$\theta$} ; 
   \edge[dashed, ->] {M}{rho};

%\edge{gamma}{M}
%\edge{delta}{M}
\edge{M}{nu}
%\plate{}{(gamma)(delta)(M)}{$\infty$}
\edge{meanGlobal}{X}
\edge{rho}{nu}
\edge{nu}{Y}
\edge{eta}{X}
\edge{etad}{X}
\edge{sigmaGlobal}{X}
 \edge {Y} {X}
 \edge{zeta}{X}
 \edge{Z}{X}
 \edge{sigma}{X}
 \edge{theta}{Z}
 \edge{alpha}{eta}
 \plate{etaT}{(etad)}{$\vert \mathcal{T}_d \vert$}
 \plate{etaTD}{(etaT)}{$|Cat|$}
 \plate{}{(meanGlobal)(sigmaGlobal)}{$\vert Num \vert$}
 \plate{plateNY}{(nu)(Y)}{$D = |Num| + |Cat|$}
 \plate{plateEta}{(eta)(alpha)}{$\vert \mathcal{T}_d \vert$}
 \plate{plateCat}{(plateEta)}{$\vert Cat \vert$}
 \plate{plateZeta}{(zeta)(sigma)}{$\vert Num \vert$}
 \plate{}{(plateNY)(plateCat)(plateZeta)}{$\infty$}
 %\plate{}{(mu)(nu)(Y)}{$D$}
 \plate{plateX}{(X)}{$D$}
 \plate{plateZ}{(Z)}{$\infty$}
\plate{plateZX}{(plateZ)(plateX)}{$N$}
 %\plate{plate1}{(plateEta)(plateZeta)(Y)}{$\infty$}
 
%\plate{}{(nu)(plate1)(X)}{$D = \vert Cat \vert + \vert Num \vert$}

 
 
 \end{tikzpicture}
 
  % Factors
%  \factor[above=of X]     {X-f}     {Multi} {} {} ; %
%  \factor[above=of T]     {T-f}     {left:Multi} {} {} ; %
%  \factor[above=of theta] {theta-f} {left:Dir} {} {} ; %

  
  %\node[const, above=of phi]  (aphi) {$\alpha_\phi$}; %

  %\factor[above=of phi] {phi-f} {right:Dir} {} {} ; %

%%  \factoredge {theta}  {T-f}     {T} ; %
%%  \factoredge {atheta} {theta-f} {theta} ; %
%%  \factoredge {phi}    {X-f}     {X} ; %
%%  \factoredge {aphi}   {phi-f}   {phi} ; %
%%
%%  \gate {X-gate} {(X-f)(X-f-caption)} {T}
%%
%%  \plate {plate1} { %
%%    (X)(X-gate) %
%%    (T)(T-f)(T-f-caption) %
%%  } {$\forall 1 \leq i \leq n_d$}; %
%%  \plate {} { %
%%    (plate1) %
%%    (theta)(theta-f)(theta-f-caption) %
%%  } {$\forall d \in \mathcal{D}$} ; %
%%  \plate {} { %
%%    (phi)(phi-f)(phi-f-caption) %
%%  } {$\forall t \in \mathcal{T}$} ; %
%%
%%\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 


==> conclusions.tex <==
\section{Conclusions}

Our work provides a game theoretic extension of structured prediction and generalizes prior work on learning graphical or aggregative games from data. We showed convergence guarantees for alternative aggregative dynamics of the game. Empirical results are encouraging in terms of uncovering meaningful strategic interactions from data. 

A number of extensions are possible. The game dynamics used for learning in our setup differs slightly from those analyzed theoretically, and these could be reconciled. As the equilibrium is obtained approximately, analogously to structured prediction with approximations, we can study self-stabilization properties of the approximation, i.e., whether the approximation improves through learning. The utilities in our game can be generalized substantially without precluding gradient-based learning though the analysis of game dynamics becomes more challenging. The strategic interactions between the players, even if expressed in an aggregative form, can be also made and learned in a context dependent manner to capture richer realistic scenarios.  

==> experiments.tex <==
\begin{figure}
%\centering
    \begin{subfigure}[b]{0.5\textwidth}            
            \includegraphics[trim=0cm 0.3cm 0cm 0.5cm,clip, width=\textwidth]{MapMultiplePos.png}
            \caption{Positive influence}
            \label{fig:UNGAa}
    \end{subfigure}%
    ~
     %add desired spacing between images, e. g. ~, \quad, \qquad etc.
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.5\textwidth}
           % \centering
            \includegraphics[trim=0cm 0.3cm 0cm 0.5cm,clip,width=\textwidth]{MapMultipleNeg.png}
            \caption{Negative influence}
            \label{fig:UNGAb}
    \end{subfigure}
    \caption{{\bf UNGA structure recovery with LAGs}:  Incoming arrows show (a) 2 countries with the most positive influence quantified by  $\hat{w}_{ij}$, and (b) 2 countries with the most negative influence on each country $i$. The estimated connections are largely consistent with the expected alignments of the countries.
In particular,  (a) shows that the two blocs (indicated by red and blue nodes) are well segregated from each other in that very few edges cross from one bloc to another.  More interesting alignments are revealed, e.g., every node in the red has a directed path from Russia, and likewise every node in the blue is reachable from USA thereby showing the strong influence of these countries.  Additionally, (b) reveals, e.g., that a significant fraction of negative connections emanate from or end at Israel and USA on one side and the red nodes on the other.}\label{fig:UNGA}
\end{figure} 


\begin{figure*}[t]
%\centering
 \input{RehnquistCourtQuant}
 \caption{{\bf Quantitative comparison with prior methods}:  (a), (b), and (c) show the structures estimated by LAG, local aggregative game [11], and tree structured potential game [10] on US Supreme Court data.  Since only the conservatives (red nodes) and liberals (blue nodes) are known to influence the moderates (green nodes) and not vice-versa,  we define a {\em correct edge} to be one that either (1) connects two red nodes, two blue nodes, or two green nodes in any direction, or (2) goes outward from a red node or a blue node into a green node. One natural way to quantify the quality of recovery is to compute the fraction of correct edges. All 14 edges recovered by LAG are correct, and therefore its recovery score is maximum possible, i.e., 1. On the other hand, Local AG [11] gets edges \{(O, R), (O, T), (O, Sc), (O, B), (K, Sc), (K, T)\} wrong for a score of only 16/22, i.e. 0.73. Finally, the Potential game [10] only recovers undirected edges, which we treat with bidirectional edges.  Thus, [10] recovers 16 edges out of which it makes mistakes on \{(O, So), (St, R), (R, St), (St, Sc), (Sc, St)\}, and  thus registers a score of  11/16, i.e., 0.69.  One could also restrict to only top 14 edges with maximum weights  for each method. We color the remaining edges in red. The scores for models under this restriction are: {\bf LAG = 1, Local AG = 0.64, Potential game = 10/14 = 0.71}.} \label{fig:RehnquistCourt}  %On the other hand justices with the most positive and the most negative influence, quantified by $\hat{w}_{ij}$, on each Justice $i$. The estimated connections are consistent with the known jurisprudence of the Court. In particular,  (a) shows the coherence between the conservatives on the left (shown in red), that between the liberals on the right (shown in blue), and the separation between these ideologies with the moderates in the center (shown in green). Likewise, (b) shows all the negative connections are between the blocks. Note that the moderates (K) and (O) have  only incoming connections in both  (a) and (b), unlike the liberals and the conservatives. This emphasizes, in particular, that the moderates espouse a centrist viewpoint and do not exercise strong influence on the others, positive or otherwise.} \label{fig:RehnquistCourt}
\end{figure*} 
\vskip -0.15in

\begin{figure}
%\centering
    \begin{subfigure}[b]{0.45\textwidth}            
            \includegraphics[width=\textwidth]{MapAdversarialPos.png}
            \caption{Positive Influence}
            \label{fig:NoContexta}
    \end{subfigure}%
    ~
     %add desired spacing between images, e. g. ~, \quad, \qquad etc.
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.45\textwidth}
            %\centering
            \includegraphics[width=\textwidth]{MapAdversarialNeg.png}
            \caption{Negative Influence}
            \label{fig:NoContextb}
    \end{subfigure}
    \caption{{\bf Effect of randomizing initial strategies}. Games such as \cite{GJ2017} ignore the context altogether in the modeling of strategic settings. We show the potential limitations of such modeling by providing the results with an alternate setting where noisy transformed contexts are provided to the players, and the parameters pertaining to the transformations are estimated by adversarial training.  (a) and (b) are the counterparts of the corresponding plots in Fig. 1 with this modification. Some significant anomalies are seen in the recovered structure. For instance, in (a), South Korea has a high positive influence on North Korea which, in turn, has a positive effect on Japan!  Similarly, in (b), there are several negative connections amongst the members in blue, including the NATO members that closely associate with each other. Since this setting provides strictly more information than one without context, our results elucidate the difficulty in recovering game structures that forego the contextual information. }\label{fig:NoContext}
\end{figure} 




\section{Experiments}
We now provide detailed empirical evidence that LAGs meaningfully estimate the strategic influences on two real world data corresponding to  (a) United Nations General Assembly (UNGA)  and (b)  US Supreme Court. We implemented the neural architecture described in the previous section, and fixed $k = 5$ and $\alpha = 0.1$. All our models were trained in batches of size 200 for 1000 epochs and used the default parameter settings of the RMSprop optimizer in the PyTorch library.  

Additionally, we provide results of our experiments that illustrate the benefits of modeling context in LAGs over methods such as \cite{GJ2017}. Toward that goal, we conjured an alternate setting, where the players do not observe the true contexts $x$ but the perturbed contexts $\tilde{x} =\epsilon + \phi(W_2\phi(W_1x + b_1) + b_2) \in \mathbb{R}^d$, such that the linear transformations $W_1 \in \mathbb{R}^{d_1 \times d}$ and $W_2 \in \mathbb{R}^{d \times d_1}$ with the bias terms are additional parameters to be learned,  $\epsilon$ is sampled from isometric $d$-dimensional Gaussian noise, and  $\phi$ is a nonlinearity (e.g. rectified linear unit).  The (hypothetical) players then undergo dynamics under these contexts using the same architecture as for LAGs and reach their $k$-step strategies that can be sampled to yield the configurations $\tilde{y}$. The role of $\epsilon$ is to encourage randomness in the initial strategy selection for a given $x$. Thus, in order to harbor any hopes for meaningful estimation in the absence of contextual information, we should at least be able to recover the parameters in this more amenable generative setting that provides strictly more information in terms of $\tilde{x}$. 

%, and thereby model the uncertainty inherent in strategic game settings that overlook the context.
In this alternative setting, we sampled $\tilde{y}$ from the continuous $k$-step strategies via the Gumbel-Softmax approximation \cite{JGP2017}. %and encoded it as  a concatenation of the respective one-hot representations of the sampled actions of the players.  
We let the feedback from an additional {\em discriminator} adversarial one layer neural network $D$  to guide the parameter estimation process. The discriminator \cite{G2014} provides a loss signal in $[0, 1]$ to tell the true configurations $y$ from the generated configurations $\tilde{y}$, and thus one can update the parameters $W_1, W_2, b_1, b_2$ as well as the type and aggregator weights that together form our generator $G$.  Thus, the objective is
$$\min_{G} \max_{D} \mathbb{E}_{(x, y)} \mathbb{E}_{\epsilon} \log(1 - D(\tilde{y}(\tilde{x}))) + \log(D(y)),$$ 
which can be optimized using alternate generator and discriminator gradient update steps with rate $\kappa$ via a standard GAN procedure \cite{G2014, MO2014}. Specifically, for our experiments we found that training was stable with an architecture using the following settings: $\kappa = 0.01$ and  $d_1 = 10$.  

To account for randomness in training, we executed each model with 5 independent initializations and averaged the parameters across these runs. We characterize the influence of other players $j$ on player $i$ in terms of the ordering of the estimated average values from the most positive to the most negative.    

\subsection{United Nations General Assembly (UNGA) Data}
The UNGA data consists of the roll call votes of the member countries on the resolutions considered in the UN General Assembly. Each resolution is a textual description that provides a context while the votes of the countries on the resolution pertain to a configuration.  We compiled data on all resolutions in UNGA since 1992 to understand the interactions of member nations since the dissolution of the Soviet Union.  We considered 25 countries for our experiments that have dominated the international, and in particular the United States (USA) politics. These countries are generally known to belong to one of the two blocs: pro-USA countries, namely, Australia (AUS),  Canada (CAN), France (FRA), Germany (GER), Israel (ISR), Italy (ITA), Japan (JPN), South Korea (KOR), Norway (NOR), Ukraine (UKR); and the others, namely,  Afghanistan (AFG), Belarus (BLR), China (CHN), Cuba (CUB), Iran (IRN), Iraq (IRQ), Kazakhstan (KAZ), Mexico (MEX), Pakistan (PAK), Philippines (PHL), North Korea (PRK),  Russia (RUS), Syria (SYR), Venezuela (VEN) and Vietnam (VNM).  We used pretrained GLoVe word embeddings to represent each context $x^m  \in \mathbb{R}^{50}$ as the mean embedding of the words in its resolution. Each vote was interpreted to take one of the three values: 1 (yes), 2 (absent/abstain), or 3 (no), and we represented $y^m$ as a 26-dimensional vector.  Fig. \ref{fig:UNGA} shows the structure estimated by our method, i.e., the weights $\hat{w}_i$ learned for each country $i$. The weights $\hat{w}_{ij}, j \neq i$ have a natural interpretation in terms of influence: the more positive $w_{ij}$ is, the more positive the influence of $j$ on $i$. A similar connotation holds for the negative weights. To avoid clutter and aid visualization, we disentangle the positive connections from the negative connections, and only depict the most influential connections for either case. As shown in Fig. \ref{fig:UNGA}, our method yields a structure that is qualitatively meaningful.  We also vectorized the learned type parameters $\theta_i$ and computed the cosine similarity with the other players. Fig. \ref{fig:UNGAType} provides evidence that the type parameters for members in the same bloc turned out to be similar.  Finally, we demonstrate the significance of modeling context  via results with the transformed context setting. Evidently, as Fig. \ref{fig:NoContext} shows, several spurious connections arise that undermine the estimation procedure. This highlights a major pitfall of the prior works, such as \cite{GJ2017}, that do not leverage context in the estimation process.  %The details are provided in the captions of these figures.       

\begin{figure}
%\centering
    \begin{subfigure}[b]{0.4\textwidth}            
            \includegraphics[trim=0cm 0.3cm 0cm 0.55cm,clip,  width=\textwidth]{MultipleTypePos.png}
            \caption{Type similarity}
            \label{fig:TypePos}
    \end{subfigure}%
    \qquad \qquad
    \begin{subfigure}[b]{0.4\textwidth}            
            \includegraphics[trim=0cm 0.3cm 0cm 0.78cm,clip,  width=\textwidth]{MultipleTypeNeg.png}
            \caption{Type dissimilarity}
            \label{fig:TypeNeg}
    \end{subfigure}%
 \caption{{\bf UNGA type recovery with LAGs}:  Incoming arrows show (a) 2 countries with the highest cosine similarity $\hat{\theta}_{i}^{\top} \hat{\theta}_j/(||\hat{\theta}_i||~||\hat{\theta}_j||)$ (black edges), and (b) 2 countries with the most negative influence (magenta edges), to each country $i$. Types determine the initial strategies, and therefore, we would expect the type vectors to be reasonably aligned with the final outcomes. The estimated connections in (a)  and (b) are indeed largely consistent with our intuition. 
 A careful look at (b) reveals two interesting negative connections from US to South Korea, and from Israel to Norway, although they usually identify with the same bloc. Indeed, during the considered period (1992-2017), Israel and Norway have had heightened tensions over the recognition of Hamas by Norway, and  likewise US and South Korea  have sparred over beef as well as dumping of formaldehyde in the Han river.}\label{fig:UNGAType}
\end{figure}



    
%     %add desired spacing between images, e. g. ~, \quad, \qquad etc.
%      %(or a blank line to force the subfigure onto a new line)
%    \begin{subfigure}[b]{0.4\textwidth}
%            %\centering
%            \includegraphics[width=\textwidth]{TypeNoContextPos.png}
%            \caption{No context}
%            \label{fig:TypeNoContextPosb}
%    \end{subfigure}
%    \caption{Type Networks: Positive Influence}\label{fig:TypeNoContextHigh}
%\end{figure} 
%
%\begin{figure}
%%\centering
%    \qquad \qquad
%     %add desired spacing between images, e. g. ~, \quad, \qquad etc.
%      %(or a blank line to force the subfigure onto a new line)
%    \begin{subfigure}[b]{0.45\textwidth}
%            %\centering
%            \includegraphics[width=\textwidth]{TypeNoContextNeg.png}
%            \caption{No context}
%            \label{fig:TypeNoContextNegb}
%    \end{subfigure}
%    \caption{Type Networks: Negative Influence}\label{fig:TypeNoContextLow}
%\end{figure} 

%We considered the Rehnquist Court since it is known to be the longest stretch in US Supreme Court history to have been served by the same 9 justices.
\subsection{US Supreme Court Data}
For our second data, we included all the cases from the longest serving US Supreme Court ever, the {\em Rehnquist Court}, during the period 1994-2005 that had votes documented for all the 9 justices.  Justices Rehnquist (R), Scalia (Sc),  and Thomas (T) represented the conservative side; Justices Stevens (St), Souter (So), Ginsburg (G), and Breyer (B) formed the liberal bloc; and Justices Kennedy (K) and O'Connor (O) followed a largely moderate ideology. Our contexts comprise of 38 binary features resulting from several categorical fields that characterize the specifics of the appeal, namely, {\em issueArea}, {\em jurisdiction}, {\em threeJudgeFdc}, {\em lcDisagreement}, {\em certReason}, {\em lcDisposition},  {\em lcDispositionDirection}, {\em term}, {\em authorityDecision1}, {\em authorityDecision2}, {\em lawType},and {\em caseOriginState}.  The original data also contains the votes, each of which takes a value in the set $\{1, 2, 3, 4, 5, 6, 7, 8\}$, where the values 1, 3, 4, and 5 denote alignment with the majority ruling, 2 indicates dissent, and the remaining votes have a more complex interpretation. We treated these three categories as 1 (yes), 2 (no), and 3 (complex) to obtain our 3-dimensional configurations.  Fig. \ref{fig:SupremeCourt} shows that how our method yields a structure that is consistent with the known jurisprudence of the Rehnquist Court. %

\begin{figure}
%\centering
    \begin{subfigure}[b]{0.45\textwidth}            
            \includegraphics[width=\textwidth, trim=0cm 0.3cm 0cm 0.78cm,clip,  width=\textwidth]{MultipleJusticePosUnWeighted.png}
            \caption{Positive influence}
            \label{fig:SupremeCourta}
    \end{subfigure}%
    \qquad 
     %add desired spacing between images, e. g. ~, \quad, \qquad etc.
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.4\textwidth}
           % \centering
            \includegraphics[width=\textwidth, trim=0cm 0.1cm 0cm 0cm,clip,  width=\textwidth]{MultipleJusticeNegUnWeighted.png}
            \caption{Negative Influence}
            \label{fig:SupremeCourtb}
    \end{subfigure}
   \caption{{\bf Supreme Court structure recovery with LAGs}:  (a) and (b) show, respectively, justices with the most positive and the most negative influence, quantified by $\hat{w}_{ij}$, on each Justice $i$. The estimated connections are consistent with the known jurisprudence of the Court. In particular,  (a) shows the coherence between the conservatives on the left (shown in red), that between the liberals on the right (shown in blue), and the separation between these ideologies with the moderates in the center (shown in green). Likewise, (b) shows all the negative connections are between the blocks. Note that the moderates (K) and (O) have  only incoming connections in both  (a) and (b), unlike the liberals and the conservatives. This emphasizes, in particular, that the moderates espouse a centrist viewpoint and do not exercise strong influence on the others, positive or otherwise.  Additionally, the type parameters estimated by our method are along the expected lines (we omit the details for brevity). \newline \newline  Clearly, our results with both the datasets underscore the efficacy of LAGs in encapsulating an extremely rich class of finite games, and the concomitant paraphernalia in unraveling the behaviors from data arising in diverse strategic settings. Unlike prior works, these games are cast in a repeated incomplete information setting, may handle arbitrary voting data, and do not impose any local consistency restrictions on data. In summary, we 
contribute a novel conceptual game theoretic framework that has rigorous theoretical foundations and extremely significant practical implications.} \label{fig:SupremeCourt}
\end{figure} 





==> introduction.tex <==
%!TEX root = main.tex

\section{Introduction}
Structured prediction methods \cite{LMP2001, TCK2003, TJHA2005, NL2011} typically operate on parametric scoring functions whose maximizing assignment is used as the predicted configuration. Since the parameters can be learned directly to maximize prediction accuracy, often via surrogate losses, the methods have been very successful across areas. They continue to be developed in terms of models and inferential strategies \cite{CSYU2015} along with the associated theory \cite{GRSY2015, LHG2016, CKMY2016, OBL2017}. 

Not all structured observations can be naturally modeled as extrema of scoring functions. When the output variables correspond to actions or strategies adopted by individual players in a game, the observed configuration is an equilibrium rather than a maximizing assignment. Indeed, game equilibria do not generally correspond to any common scoring function. Our goal in this paper is to provide the analogous prediction framework tailored for games. We do so in a manner that uncovers as a by-product of strategic interactions between the players. 

Our structured prediction approach produces a mixed-strategy equilibrium as the predicted outcome in response to contextual cues. We focus on aggregative games (e.g., \cite{GJ2017}) that shield each player from information about a particular neighbor in an underlying (to be learned) digraph while retaining the ability of players to react to aggregated versions of their neighbors' actions. Several aggregators are possible and we consider two of them: {\em active aggregator} (AA) and the {\em passive aggregator} (PA) that differ in terms of the amount of feedback provided. We model the impact of context as an infusion of private information to each player (player types), incorporated into their utilities and the initial strategy profiles. The game dynamics plays a key role in our approach as it serves to isolate a particular mixed strategy equilibrium as the predicted configuration. To this end, we introduce two kinds of game dynamics, based on derivative fictitious play and gradient play \cite{B1951, R1951, FK1993, SA2005}, for both aggregators and provide a detailed characterization of the conditions under which the players converge to a mixed strategy Nash equilibrium. We demonstrate the benefits of our approach on strategic structure recovery on two real voting datasets, namely, the United Nations General Assembly and the United States Supreme Court that comprise discrete votes with more than two alternatives. 

Our work extends and generalizes previously published results on learning games from data. For example, methods in \cite{GJ2016, GJ2017} model each observed configuration as a (nearly) pure strategy Nash equilibrium of an appropriately defined repeated graphical game \cite{KLS2001, KM2002} but do not incorporate context nor the game dynamics. The focus on pure strategies also restricts their applicability since pure strategy Nash equilibria do not exist in a wide class of games \cite{TV2007}. Moreover, the key estimation setups in these approaches are inherently combinatorially hard, forcing the use of approximate methods. Finally, our theoretical analysis brings together tools from control theory, dynamical systems, and stochastic approximation theory \cite{B2008, KY2003, B1997, BHS2005, BHS2006, BPP2013, CL2003, HRUNH2017}, and might be of independent interest.



\iffalse
Structured prediction methods \cite{LMP2001, TCK2003, TJHA2005, NL2011} typically learn a parametrized map $\phi_w: \mathcal{X} \times \mathcal{Y} \to \mathbb{R}$ such that $\tilde{y} \in \arg\!\max_{y \in \mathcal{Y}} \phi_w(\tilde{x}, y)$ for a given context $\tilde{x} \in \mathcal{X}$ and configuration $\tilde{y} \in \mathcal{Y}$.  These methods have enjoyed great success in diverse domains, and thus continue to generate interest \cite{CSYU2015, GRSY2015, LHG2016, CKMY2016, OBL2017}. However, alternative models are required for settings that entail strategic interactions among multiple non-cooperative entities and lead, at best, to {\em locally} stable configurations \cite{GJ2016, GJ2017, GH2017}.  

A central idea underlying the methods in \cite{GJ2016, GJ2017} is to model each observed configuration as  a (nearly) pure strategy Nash equilibrium of an appropriately defined repeated graphical game \cite{KLS2001, KM2002}. This abstraction severely restricts their applicability since pure strategy Nash equilibria do not exist in a wide class of games \cite{TV2007}.   Additionally, they presume that each player knows exactly all the information about the other players. This assumption is clearly unrealistic in most real world, incomplete information scenarios, where the players have some private {\em type} information that is hidden from the others. Moreover, the learning formulations proposed in these works are combinatorially hard, leading to computational bottlenecks. Besides, these formulations are cast in the setting of only binary data, and it is not clear if they can handle arbitrary discrete data. Finally, these methods either ignore altogether the context and the dynamics that might have resulted in equilibria \cite{GJ2017}, or provide estimation algorithms that are completely disentangled from the dynamics \cite{GJ2016}.   

 We introduce a new class of games, {\em latent aggregative games} (LAGs), to address all these issues.  In these games, the payoff of each player depends on its private information or {\em latent type} that depends on a given context, its strategy, and the aggregate strategy of its neighbors on an underlying  digraph. The players play a repeated game with their neighbors in an incomplete information setting, where they do not know the types of other players and their individual strategies. We consider two different aggregators, the {\em active aggregator} (AA)  and the {\em passive aggregator} (PA), depending on the amount of feedback provided by the aggregator.   We introduce two kinds of dynamics, based on derivative fictitious play and gradient play \cite{B1951, R1951, FK1993, SA2005}, for both these settings and provide a detailed characterization of the conditions under which the players converge to a ({\em mixed strategy}) Nash equilibrium.  We model each data configuration $y$ as a discrete random sample of the equilibrium reached by our dynamics under context $x$.  Thus these configurations do not necessarily pertain to Nash equilibria (pure or otherwise). Since a mixed strategy Nash equilibrium is guaranteed to exist in {\em any} finite game \cite{N1951}, and we do not impose the pure strategy equilibrium constrains, our treatment significantly extends the scope of the strategic settings that could be learned. %Additionally, we do not need to impose any convexity, submodularity or Lipschitz assumptions on the payoff functions as required by \cite{GJ2017} to ensure the existence of pure equilibria.
 
 
   We introduce a neural architecture, inspired by our dynamics, to estimate the types of the players and the underlying structure of the game from strategic data. Finally, we go beyond the binary vote assumption and demonstrate the benefits of our approach via meaningful structure recovery on two real voting datasets, namely, the United Nations General Assembly and the United States Supreme Court that comprise discrete votes with more than two alternatives. 

% Specifically, we formulate the discrete time evolution of our game as a noisy discretization of a limiting ordinary differential equation (ODE) that it tracks asymptotically under standard assumptions. Then, under the prescribed dynamics, players would converge with positive probability to an asymptotically stable Nash equilibrium of the game.
\fi
  
